Stimuli-Sensitive Hawkes Processes for Personalized Student Procrastination Modeling

Student procrastination and cramming for deadlines are major challenges in online learning environments, with negative educational and well-being side effects. Modeling student activities in continuous time and predicting their next study time are important problems that can help in creating personalized timely interventions to mitigate these challenges. However, previous attempts on dynamic modeling of student procrastination suffer from major issues: they are unable to predict the next activity times, cannot deal with missing activity history, are not personalized, and disregard important course properties, such as assignment deadlines, that are essential in explaining the cramming behavior. To resolve these problems, we introduce a new personalized stimuli-sensitive Hawkes process model (SSHP), by jointly modeling all student-assignment pairs and utilizing their similarities, to predict students' next activity times even when there are no historical observations. Unlike regular point processes that assume a constant external triggering effect from the environment, we model three dynamic types of external stimuli, according to assignment availabilities, assignment deadlines, and each student's time management habits. Our experiments on two synthetic datasets and two real-world datasets show a superior performance of future activity prediction, comparing with state-of-the-art models. Moreover, we show that our model achieves a flexible and accurate parameterization of activity intensities in students.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> related-work.tex <==
\noindent
\textbf{Hawkes process and modeling scenarios}
% Hawkes process, as a popular family of temporal point process, has long been used in sequential data modeling across a wide range of scenarios, such as social and information networks analysis~\cite{zhao2015seismic,Farajtabar2017}, recommendation system~\cite{Du2015,wang2019modeling}, financial applications~\cite{Linderman2014,BacryBACRY2018}, and crime detection~\cite{Mohler2013,Egesdal2010}. 
%------------------intro of hawkes--------
% As a family of point process, one of the merits of Hawkes process comparing with other popular point processes such as Poisson process, is its ability to capture the self-exciting nature of the sequences, i.e. past activities could trigger future ones.
% As a result, Hawkes process has long been used across a wide range of scenarios where self-exciting nature of the sequences is frequently observed. Examples including social and information networks analysis~\cite{zhao2015seismic,Farajtabar2017}, recommendation system~\cite{Du2015,wang2019modeling}, financial applications~\cite{Linderman2014,BacryBACRY2018}, and crime detection~\cite{Mohler2013,Egesdal2010}. 

% To capture the self-excitation of a process, Hawkes process models the combined intensity that comes from two types of events from the sequence: the arrivals of immigrants (i.e. the events that are triggered externally) are modeled via a base rate function that describes the influence of the external stimuli to the sequence, and offspring (i.e. the events that are triggered internally by the history) are modeled via a excitation function that describes the dependency between past events and the future ones. 
% In the literature, efforts have been made in both directions by proposing state-of-the-art base rate functions and the excitation functions to better characterize the intensity of the arrivals of the events. 

%------------------customized base----------
When modeling base rate, t
Tradition Hawkes models parameterize the base rate of a sequence as a constant, which makes it difficult to capture the varying characteristics of activity jumps across time~\cite{wang2019modeling}. 
To tackle this problem, some customized parameterization have been proposed based on the problems at hand. 
For example, Rizoiu et al. proposed to model a YouTube video watching history as a Hawkes process, and proposed to use the number of shares of a video on YouTube scaled by a constant to be the base rate~\cite{rizoiu2017expecting}. 
In a similar application, Ding et al. modeled the base rate via power law function, based on the intuition that the chance of a video being watched by new users since it's published decays very quickly over time ~\cite{ding2015video}.
In another example, Bao et al. proposed to use a sinusoidal function to capture the periodical rise-and-fall patterns of user activities on social media~\cite{bao2016modeling}. 
These customized base rate functions even though could possible better describe the data at hand, the model capacity may vary when a new scenario is adopted. For example, the number of times a video is shared on YouTube is not a relevant factor in modeling user retweeting on Twitter or students' interactions with online course materials.
%----------------customized kernel-------------
Another important component of sequence intensity modeling is the excitation function. The most common choices of parameterization of excitation kernel in most traditional Hawkes models are exponential (e.g.~\cite{Du2015}), Gaussian~(e.g. \cite{xu2016learning}), and power-law distribution(e.g. \cite{mishra2016feature}). The effect of self-excitation is usually characterized by the linear addition of all previous events up to a certain time $t$.
More recently, neural Hawkes models have been proposed to allow higher model capacity for learning arbitrary and nonlinear distributions of the history~\cite{du2016recurrent,mei2017neural,xiao2017modeling}. For example, Du et al. proposed to use RNN to model the arrival times of a given sequence and characterized the intensity as a function of the embedded hidden cell representation, thus could potentially capture more complicated sequence dynamics compared to traditional Hawkes models~\cite{du2016recurrent}. 
% Such RNN-based models predict future time after time $t$ based on a completely observed history unfolded up to time $t$. 
Even though such neural based Hawkes models allow for less bias and more flexibility than the traditional parametric models, they do not provide meaningful interpretations of the activity arrival patterns, which could be important to some scenarios such as procrastination analysis in education domain.

In terms of the applications of sequential data modeling via Hawkes models, in the literature, there are two types of modeling methods: the majority of the state-of-the-art Hawkes models treat each individual sequence as an independent input, in other words no relationship among the sequences are assumed. 
As a result, a complexity that is proportional to the size of the data can usually be achieved. 
On the other hand however, since all sequences are assumed to be i.i.d., sequences without any observed history need either to be discarded from the study, or can not obtain personalized prediction, meaning that they have to share the parameters that are learned from the sequences from the training data. 
To tackle this problem, the second modeling methods model all sequences jointly by assuming underlying similarity among the sequences. 
For example, Du et al. modeled a user-item pair, i.e., the interactions of a user to an item they purchased as a Hawkes process, at the same time, their model imposed a low rank constraint on the matrix representation of the Hawkes process parameters~\cite{Du2015}. 
As a result, even the user-item sequences where there is no observations available can be inferred based on their similarity to the others. 
Other similar approaches have also been proposed to better measure the similarity among sequences by using auxiliary features~\cite{He2015,Li2018,Shang2018}. 
However, auxiliary information in education domains are usually excluded from the data due to privacy concerns. The downside of these joint models is the complexity, as matrix manipulations are usually involved.



% Nevertheless, most univariate Hawkes process models assume little or no similarity or relationship between the sequences. As a result, sequences without any observed history can not obtain meaningful~\textit{personalized} predictions, meaning that their future can not be inferred unless the set of parameters learned from other sequences are used on these unseen sequences. To deal with this problem, low-rank Hawkes process models are proposed. Compared to the traditional Hawkes models mentioned above, these approaches parameterize all sequences \textit{jointly} by assuming a low-rank structure among the sequences' parameters (e.g. user-item pairs). As a result, these models are capable of inferring the future events for the sequences without historical observations by leveraging their similarity to samples that do have historical observations. 
% However, such methods usually rely on auxiliary information~\cite{He2015,Li2018,Shang2018}. 
% For example, in the recommender system setting, Shang et al. impose a local low-rank constraint on the parameter matrix to model large-scale user-item interactions by first computing user-item pairs' similarities via item features~\cite{Shang2018}. 
% % using auxiliary information, such as item features, that capture the similarity between user-item pairs~\cite{Shang2018}.
% In contrast, due to privacy constraints in our application, many educational datasets are highly anonymized and auxiliary information is scarce in them.
% Consequently, having a model that does not require such information is valuable in our context. Among these low-rank Hawkes models, the most relevant work to ours is low-rank Hawkes processes proposed by Du et al.~\cite{Du2015}, to capture user-item interaction and recommend items ``at the right moment'' without using any auxillary information.

% Other related Hawkes models that consider the correlation or possible dependence among the sequences are multivariate Hawkes model~\cite{Zhou2013,Luo2015,Bacry2015,Lemonnier2017,shang2019geometric,wu2020modeling}. 
% However the focus of such models is to capture the mutual-excitation between sequences, i.e., the causal effect of one sequence to another. 
% For example, in social networks, one can assume that, activities from different social network platforms can trigger each other. 
% In our application of modeling students' procrastination behavior, neither a students' activity triggers another student's activity, nor the deadline of one assignment triggers the activities that are related to another assignment.
% % Since the assignments are not parallel, activities for each assignment are only triggered by the same assignment's deadline.
% % Also, since students do not work in teams and are not in a social setting, studying activities of each student can only be the offspring of the same student's past activities.
% Hence, we build our model based on the uni-variate Hawkes process.

\noindent
\textbf{Procrastination Modeling in Education Domain}
As there is no quantitative definition for procrastination behavior, in most of the recent educational data mining literature, procrastination-related behavior has been summarized by curating time-related features from student interactions in the course.
These studies aim to evaluate the relationships between these time-related features with student performance and do not model temporal aspects of procrastination~\cite{Baker2016,Cerezo2017,Kazerouni2017,agnihotriprocrastination}.
For example, Asarta et al. examined the students log data from an online course use measures such as anti-cramming, pacing, completeness etc.~\cite{asarta2013access}. However, such methods are static and can not describe students varying behaviros over time.
%Capturing the temporal aspects of procrastination, such as activity intensity or burstiness, has been attempted in a few numbers of recent works~\cite{Backhage2017,Park2018}.
For another example, Park et al. classify students to procrastinators vs. non-procrastinators by formulating a measure via a mixture model of per-day student activity counts during each week of the course~\cite{Park2018}. But, it cannot model non-homogeneously spaced deadlines in a course.

As none of these models consider the timing of students activities, they are not able to predict~\textit{when} the future activities will happen.
Sequential data modeling via point process could potentially deal with this limitations, however has not been applied to procrastination modeling until recently. 
To the best of our knowledge, the most related attempt that is comparable to ours has been made in~\cite{Yao2020}, where Yao et al. modeled each student's activities sequence as a Hawkes process and relates procrastination to the mutual excitation among activity types.
This work does predict student's unseen activities, rather, a procrastination measure was proposed based on the learned parameters that have shown to be better correlated with students grades than conventional delay measure.
%Since this model is the closest research on procrastination modeling to our work,
We use this model, called EdMPH, as one of our baselines.
% , even though it uses a multi-variate Hawkes model.
